Exploring the Limits of ChatGPT in Software Security Applications

Large language models (LLMs) have undergone rapid evolution and achieved remarkable results in recent times. OpenAI's ChatGPT, backed by GPT-3.5 or GPT-4, has gained instant popularity due to its strong capability across a wide range of tasks, including natural language tasks, coding, mathematics, and engaging conversations. However, the impacts and limits of such LLMs in system security domain are less explored. In this paper, we delve into the limits of LLMs (i.e., ChatGPT) in seven software security applications including vulnerability detection/repair, debugging, debloating, decompilation, patching, root cause analysis, symbolic execution, and fuzzing. Our exploration reveals that ChatGPT not only excels at generating code, which is the conventional application of language models, but also demonstrates strong capability in understanding user-provided commands in natural languages, reasoning about control and data flows within programs, generating complex data structures, and even decompiling assembly code. Notably, GPT-4 showcases significant improvements over GPT-3.5 in most security tasks. Also, certain limitations of ChatGPT in security-related tasks are identified, such as its constrained ability to process long code contexts.

==> arxiv_backup/intro_backup.tex <==
\section{Introduction}
\label{sec:introduction}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.40\textwidth]{figures/fig1.png}
    \caption{Categories of ChatGPT-based software security tasks and open research questions covered by this work.}
    % https://docs.google.com/drawings/d/1LGKQrxxfEtoZzB68ogmdQmFQt-vP0lslRgxAS3P2pLs/edit
    \label{fig:category_chart}
\end{figure}


The recent breakthrough of large language models (LLMs) is a revolution of the research of natural language processing (NLP).
Since the invention of neural networks back in 1980s~\cite{ rumelhart1986learning}, NLP techniques evolves along with the development of more complex model structures. Recurrent Neural Networks (RNNs)~\cite{rumelhart1985learning,jordan1997serial}, invented in 1985, have a memory-like capacity which allows them to maintain information over time, making them particularly useful for sequential data like text. In 1997, Long Short-Term Memory networks (LSTMs)~\cite{hochreiter1997long} were invented to combat the vanishing gradient problem, which was a major issue with training RNNs on longer sequences.
In 2017, Vaswani et. al.~\cite{vaswani2017attention} proposed transformer models, which was a major breakthrough and opened the door to large complex models. Transformers do not require sequential data processing, instead, they use a mechanism called "attention" to weigh the importance of different parts of the input. This makes transformer incredibly efficient and effective for natural language processing (NLP), understanding (NLU) and generation (NLG) tasks.

Since then, industry players have invested significant efforts in training transformer-based language models with a large number of model parameters, i.e., Large Language Models (LLMs). OpenAI's Generative Pretrained Transformer (GPT) models~\cite{radford2018improving,radford2019language,brown2020language,gpt-4} are typical examples of such powerful LLMs. GPT models are pre-trained auto-regressive models that can generate text.
From the initial GPT-1~\cite{radford2018improving} released in 2018 to the latest GPT-4~\cite{gpt-4} released in 2023, the number of model parameters grows from 0.12 billion to 1 trillion. There are also other LLMs including Meta's OPT~\cite{zhang2022opt} and LLaMA~\cite{touvron2023llama}, Google's mT5~\cite{xue2020mt5} and LaMDA~\cite{thoppilan2022lamda}, etc.

Within the trend of LLMs in 2023, ChatGPT~\cite{chatgpt}, a chat bot backed by GPT-3.5 or GPT-4 models, is one of the most remarkable achievements. It gains public popularity instantly after its release with the amazingly high-quality AI-generated conversations. A large body of research~\cite{aljanabi2023chatgpt,gozalo2023chatgpt,aljanabi2023chatgpt,liu2023summary,bubeck2023sparks,azaria2022chatgpt} conduct measurement on ChatGPT and they demonstrates the strong capability of ChatGPT in a variety of tasks. The studies demonstrate that ChatGPT is able to not only generate natural languages but also generate tables or figures for data visualization~\cite{maddigan2023chat2vis,bubeck2023sparks}, solve mathematical problems~\cite{bubeck2023sparks,frieder2023mathematical}, play games~\cite{biswas2023role,tsai2023can}, assist healthcare services~\cite{sallam2023chatgpt}, search for neural network architecture~\cite{zheng2023can}, pass real-world exams~\cite{choi2023chatgpt,ryznar2023exams,newton2023chatgpt}, and more~\cite{bang2023multitask}, though limitation exists~\cite{gozalo2023chatgpt,borji2023categorical}, e.g., ChatGPT may give wrong or improper answers to certain questions.
Bubeck et. al.~\cite{bubeck2023sparks} does case studies on GPT-4's problem solving on mathematics, coding, vision, medicine, law, psychology and more. The study regards GPT-4 as an early general AI since it can achieve problem solving capabilities similar to human in many cases.
Especially, ChatGPT has an excellent performance on coding tasks~\cite{dong2023self,tian2023chatgpt,biswas2023role} as it can generate code blocks in various programming languages based on either various format of prompts such as incomplete code or description in natural languages. 
ChatGPT as a multi-purpose pretrained language model has a similar or superior performance on code generation compared with previous code-specific models.

As ChatGPT shows a remarkable performance on code generation, we naturally raise the question: Can ChatGPT be leveraged to boost software security?
In the rapidly evolving landscape of software development, the urgency to maintain and enhance software security is paramount. Security vulnerabilities, software bugs, and inefficient patching mechanisms pose significant risks, making the detection, analysis, and rectification of these issues a critical area of study.
Recent studies conducted preliminary evaluation on the use of ChatGPT on security-related tasks.
There are experiments showing that ChatGPT may generate insecure code~\cite{liu2023your,khoury2023secure}, similar to previous code generation models~\cite{pearce2022asleep}.
A number of studies found that ChatGPT can also be used to resolve insecure code with proper prompts.
Pearce et. al.~\cite{pearce2022examining} used several LLMs earlier than ChatGPT and manually written prompts to repair security vulnerabilities. These LLMs resolved part of the test cases and the repair was unstable.
Sobania et. al.~\cite{sobania2023analysis} tested code repair on ChatGPT and drew a similar conclusion on ChatGPT.
Xia et. al.~\cite{xia2023conversational} emphasized the importance of feedback on LLM-based code repair. To be specific, after the LLM returned an invalid patch, they appended the result of test cases, which indicates why the fixed code failed, to the prompt and query the LLM for a second time. The work presented the possibility to use LLMs including ChatGPT to fix general program bugs.
On the other hand, security researchers try to leverage LLMs in security tools.
Deng et. al.~\cite{deng2022fuzzing} leveraged a LLM model to mutate the inputs (i.e., code implementing deep learning networks) when fuzzing deep learning libraries.
Above works illustrate several promising cases of using LLMs in security research or engineering but the aforementioned tasks do not cover the broad software security and the latest ChatGPT is not widely tested.
To understand how much ChatGPT can help in the above security tasks, one should analyze ChatGPT's security-specific capabilities using representative test cases on a broad scope of software security tasks but such effort is in absence.

This work presents a comprehensive evaluation of the capabilities of ChatGPT in various software security tasks, as shown in \cref{fig:category_chart}, including vulnerability detection and repair, bug fixing, patching, software debloating, root cause analysis, decompilation, symbolic execution, and fuzzing. As these tasks traditionally require specialized knowledge and significant manual effort, the integration of AI-driven models like ChatGPT could greatly enhance efficiency and effectiveness in detecting and fixing software security.
For each software security task, we aim to answer a series of research questions:
\begin{itemize}
    \item Can ChatGPT understand the goal of the task?
    \item Can ChatGPT produces reasonable responses at least on the right direction?
    \item How accurate the ChatGPT's answers are?
    \item How different GPT-3.5 and GPT-4 performs?
    \item What is the limitation of ChatGPT if it cannot completely accomplish the task?
\end{itemize}
% (1) Can ChatGPT understand the goal of the task?
% (2) Can ChatGPT produces reasonable responses at least on the right direction?
% (3) How accurate the ChatGPT's answers are?
% (4) How different GPT-3.5 and GPT-4 performs?
% (5) What is the limitation of ChatGPT if it cannot completely accomplish the task?
In terms of our methdology, we collected benchmark datasets for vulnerability detection, vulnerability repair, and bug fixing and used the datasets to systematically evaluate the performance of ChatGPT on such tasks, giving quantitative results.
For other software security tasks, we created representative test cases manually or from motivating examples of related works. These test cases are designed to demonstrate a certain aspect of ChatGPT's capability that is useful for the security task.
For all experiments, we analyzed the outcomes of ChatGPT and discussed our hypothesis of ChatGPT's strength and limitations.

In general, ChatGPT demonstrates impressive capabilities in software security tasks. With proper prompting, ChatGPT can easily understand the purpose of the tasks and generate reasonable responses.
Especially, ChatGPT with GPT-4 presents impressively high accuracy by solving 92\% of vulnerability detection cases, 95\% of vulnerability repair challenges, 84\% of bug fixing cases, and most manually crafted test cases across various tasks, which is a significant improvement compared with GPT-3.5.
Surprisingly, ChatGPT is even able to decompile the assembly language at least on short programs, illustrating that ChatGPT can process software context not limited on source code.
We also identify several limitations of ChatGPT. It cannot interpret binary or hexadecimal code and is limited on long code context. Such limitations compromise the usefulness of ChatGPT in real-world software development. For instance, the accuracy vulnerability detection drops from 98\% to 66\% if ChatGPT is tested on real-world software vulnerabilities instead of synthetic programs. It is a promising research direction to address such limitations and systematically integrate ChatGPT into security-critical applications.

The remaining part of the paper is organized as follows: In the subsequent sections, we analyze ChatGPT's capabilities on different software security tasks. These tasks encompass vulnerability detection (\cref{sec:vul_detect}), vulnerability repair (\cref{sec:vul_repair}), bug fixing (\cref{sec:bug_fixing}), patching (\cref{sec:patching}), root cause analysis (\cref{sec:root_cause_analysis}), decompilation (\cref{sec:decompliation}), debloating (\ref{sec:debloating}), symbolic execution (\cref{sec:symbolic_execution}), and fuzzing (\cref{sec:fuzzing}). In \cref{sec:conclusion}, we provide a summary of our findings and discuss future research directions.

==> arxiv_backup/related_backup.tex <==
\section{Related work}

\subsection{Development of ChatGPT}

Instruct-GPT~\cite{ouyang2022training} serves as the foundational large language model aligned with human feedback, upon which ChatGPT (GPT-3.5 and GPT-4) is built. As demonstrated in~\cite{ouyang2022training}, Instruct-GPT exhibits significant improvements over GPT-3 in NLP tasks such as question answering, reading comprehension, and summarization. OpenAI further enhanced the model by incorporating Reinforcement Learning from Human Feedback (RLHF)~\cite{christiano2017deep}, resulting in the more powerful and intelligent GPT-3.5-turbo (ChatGPT). Not only does GPT-3.5 excel in these tasks, but its outputs also align more closely with human responses.
When it comes to natural language tasks, ChatGPT (GPT-3.5) showcases evident improvements compared to previous large language models. These advancements become even more apparent in GPT-4~\cite{gpt-4}. As illustrated in~\cite{gpt-4}, GPT-4 achieves remarkable success on diverse and challenging benchmarks, including more demanding academic and professional exams such as GRE, SAT, and AP exams. Surprisingly, GPT-4 demonstrates human-level performance on the majority of these exams, representing a substantial improvement over GPT-3.5. These results underscore the strong language understanding and reasoning abilities of ChatGPT (GPT-3.5 and GPT-4).

% \subsection{Evaluation of ChatGPT's Multi-task Capability}
\section{Evaluation of ChatGPT's Capability in Software Security}

Notably, ChatGPT (GPT-3.5)~\cite{chatgpt} and GPT-4~\cite{gpt-4} have opened up a highly promising avenue of research in artificial intelligence and machine learning. Numerous studies have investigated the capabilities of ChatGPT in different scenarios and tasks. Bubeck et. al.~\cite{bubeck2023sparks} demonstrates the impressive performance of GPT-4 in various categories of tasks, including coding, math, interaction with human, and so on.
The study argues that GPT-4 is already a general model that have capability comparable with human in diverse tasks.
In the realm of mathematics, Frieder et. al.~\cite{frieder2023mathematical} evaluated the ability of ChatGPT to solve advanced math problems through a question-and-answer format. Additionally, Shakarian et. al.~\cite{shakarian2023independent} evaluated ChatGPT's proficiency in solving math problems using mathematical language, employing a test dataset of 1000 math word problems (MWP).
In the field of physics, Lehnert~\cite{lehnert2023ai} took the initial steps towards examining ChatGPT's performance in comprehending complex physics problems. Their findings revealed that while ChatGPT could grasp individual physics concepts, it encountered difficulty in connecting these concepts to engage in further reasoning. Furthermore, according to~\cite{kortemeyer2023could}, ChatGPT demonstrated limited proficiency in passing physics courses based on calculus. During testing, ChatGPT exhibited many of the preconceptions and errors commonly seen in novice learners.
In the promising field of medicine, the representation of chemical substances, such as proteins or compounds, can be effectively conveyed in a linguistic form, illuminating the potential of ChatGPT in the medical domain~\cite{guo2023proteinchat}.
Tu et. al.~\cite{tu2023causal} embarked on exploring ChatGPT's ability in causal discovery for diagnosing neuropathic pain, representing an initial step in this area. Additionally, Liu et. al.~\cite{liu2023chatgpt} conducted a comprehensive investigation into drug editing using large language models and proposed ChatDrug, incorporating retrieval and feedback mechanisms to enhance its drug editing capabilities.
For ethical considerations, such as toxicity and bias related issues, OpenAI~\cite{gpt-4} revealed that GPT-4 can effectively deny almost all instances of eliciting negative behavior compared with GPT-3.5 but cannot guarantee the elimination of vulnerabilities.
Other studies~\cite{zhuo2023exploring, ray2023chatgpt} also discover potential ethical risks in ChatGPT.

Several studies attempt to connect ChatGPT or other LLMs with software security and evaluate its ability in these tasks. 
Regarding vulnerability detection, Cheshkov et. al.~\cite{cheshkov2023evaluation} conducted an evaluation of ChatGPT's ability to detect vulnerabilities in programs.
In the domain of secure code generation, Pearce et. al.~\cite{pearce2022asleep} evaluated whether Copilot~\cite{copilot} always generates secure code and concluded that Copilot generates insecure code with a high probability.
For vulnerability repair, Pearce et. al.~\cite{pearce2022examining} conducted pioneering research that assessed the capability of various LLMs on repairing vulnerable code examples. The results showed that LLMs may repair the vulnerabilities but the performance is unstable is greatly affected by prompts, vulnerability types, programming languages, etc.
For automated program repair (APR) realm, 
Sobania et. al.~\cite{sobania2023analysis} and Xia et. al.~\cite{xia2023conversational} analyzed the ChatGPT's performance in bug fixing. By providing the buggy code and optional error messages, ChatGPT is able to resolve algorithmic bugs in some cases.

However, we find that existing evaluation studies cannot answer how useful ChatGPT is for software security tasks. The reason is twofold. 
First, existing studies mainly focus on detection and repair of vulnerabilities or bugs, leaving the broad scope of software security untouched. For instance, automatic patching, debloating, decompilation, and root cause analysis can also be formulated as the generation and reasoning of code thus ChatGPT may be able to help.
Second, many studies are accomplished before the release of the latest GPT-4 thus cannot represent the state-of-the-art LLM performance.
To bridge the gap, we present a comprehensive evaluation study using the latest ChatGPT versions and considering broad software security tasks.  

\subsection{Applications Built Upon ChatGPT}

ChatGPT and GPT models are language generation models. To be specific, they accepts a text sequence as the input and produces another text sequence that is likely to take place after the input. When using such language models for tasks other than language generation, people design prompts to drive ChatGPT to understand the custom questions. For ChatGPT, the basic prompts are questions in natural languages. For instance, to ask ChatGPT to write code, we can set the input of ChatGPT as ``Can you write a program ...''.
The prompt design is critical for ChatGPT's performance as discussed in various studies~\cite{pearce2022asleep,pearce2022examining,sobania2023analysis,xia2023conversational}. Therefore, a series of research aims to improve ChatGPT's capability in certain tasks by carefully design the interaction with ChatGPT systematically. 

MM-ReAct~\cite{yang2023mm} is a framework that integrated ChatGPT with a pool of vision experts to achieve visual reasoning and action. Though ChatGPT cannot directly process images and videos, MM-ReAct used ChatGPT to intelligently choose what vision algorithm should be applied on which target. As a result, MM-ReAct can resolve complicated vision tasks that cannot be well handled by vision algorithms alone.
Visual ChatGPT~\cite{wu2023visual} also integrated vision models and ChatGPT and provided an intelligent user interface.
GP-Tutor~\cite{chen2023gptutor} leveraged ChatGPT's strong code understanding capability to explain the functionality of source code for education purposes. By integrating APIs of code editors (e.g., Visual Studio Code), GP-Tutor outperformed vanilla ChatGPT in the accuracy of explanation.
Park et. al.~\cite{park2023generative} used multiple ChatGPT instances to interact with each other and produced a world with generative agents where AI simulates the behavior of human. The study shows that the interactive system design can make ChatGPT models much stronger than the vanilla one.
% There are also numerous other intriguing and powerful applications that are combined with ChatGPT including coding~\cite{dong2023self,feng2023investigating,liu2023improving,chen2023gptutor}, multimodality~\cite{bang2023multitask, yang2023mm, wu2023visual}, automatic multitask systems~\cite{park2023generative}, education~\cite{baidoo2023education}, and environmental applications~\cite{biswas2023potential}.

Software security is paramount for maintaining safety in the information society. In this new era of large language models, the integration of these models with traditional security tasks presents a highly promising research direction.
Considerable efforts have been dedicated to addressing software bugs. In Xia et. al.~\cite{xia2023automated}, the authors evaluated the performance of automated program repair (APR) using large language models. The study demonstrated that increasing the sample size and incorporating fix template information can enhance the repair capabilities.
Moreover, in Xia et. al.~\cite{xia2023keep}, the authors utilized a conversational model with ChatGPT to fix program bugs and proposed ChatRepair, an automated conversation-driven APR approach that iteratively generates patches for bugs in programs.
Jin et. al.~\cite{jin2023inferfix} also proposed an end-to-end repair pipeline specifically tailored to address program bugs.
It is important to note that bugs and vulnerabilities are distinct concepts within the software field. 
Recognizing this, however, there has been a scarcity of LLM-based applications specifically aimed at software vulnerability at the time of writing this paper.
Therefore, further exploration of ChatGPT's potential in security-related applications, including vulnerability detection and mitigation, is warranted to advance the field of software security.
In the realm of fuzzing, Deng et. al.~\cite{deng2023large} introduced FuzzGPT, which combines large language models to automatically generate valid fuzzing input.
Furthermore, Hu et. al.~\cite{hu2023augmenting} proposed CHATFUZZ, a greybox fuzzer augmented by generative AI, demonstrating advancements in the field of fuzzing techniques.

Above ChatGPT-based applications indicate the potential of using ChatGPT in complicated and diverse tasks with certain system design. In this work, we generalize ChatGPT to various software security tasks by designing the prompts. Our design could be a baseline for future research of ChatGPT-based software security applications.
